A Symmetry-Aware Exploration of Bayesian Neural Network Posteriors

The distribution of the weights of modern deep neural networks (DNNs) - crucial for uncertainty quantification and robustness - is an eminently complex object due to its extremely high dimensionality. This paper proposes one of the first large-scale explorations of the posterior distribution of deep Bayesian Neural Networks (BNNs), expanding its study to real-world vision tasks and architectures. Specifically, we investigate the optimal approach for approximating the posterior, analyze the connection between posterior quality and uncertainty quantification, delve into the impact of modes on the posterior, and explore methods for visualizing the posterior. Moreover, we uncover weight-space symmetries as a critical aspect for understanding the posterior. To this extent, we develop an in-depth assessment of the impact of both permutation and scaling symmetries that tend to obfuscate the Bayesian posterior. While the first type of transformation is known for duplicating modes, we explore the relationship between the latter and L2 regularization, challenging previous misconceptions. Finally, to help the community improve our understanding of the Bayesian posterior, we will shortly release the first large-scale checkpoint dataset, including thousands of real-world models and our codes.

==> notations.tex <==

We summarize the main notations used in the paper in Table \ref{table:notations}.

\begin{table*}[!ht]
\renewcommand{\figurename}{Table}
\caption{\textbf{Summary of the main notations of the paper.}}
\label{table:notations}
\centering
\scalebox{0.95}
{
\begin{tabular}{ll}
\toprule
\textbf{Notations}                      & \textbf{Meaning}  \\ 

\midrule
$\mathcal{D}=\{ (\vx_i,\vy_i )\}_{i=1}^{|\mathcal{D}|}$ & The set of $|\mathcal{D}|$ data samples and the corresponding labels \\ 
\midrule
$j$, $m$, $L$ & The index of the current layer, the current subnetwork, and the number of layers\\
\midrule
$\vz^j$ & The preactivation feature map and output of the layer $(j-1)$/input of layer $j$ \\
\midrule
$\phi$& The activation function (considered constant throughout the network) \\
\midrule
$\vh^j$ & The feature map and output of layer $j$, $\vh^j = \phi (\vz^j)$ \\
\midrule
$H_j, W_j$ & The height and width of the feature maps and output of layer $j-1$ \\
\midrule
$C_j$ & The number of channels of the feature maps and output of layer $j-1$ \\
\midrule
$n_j$ & The number of parameters of layer $j$ \\
\midrule
B & The batch size of the training procedure \\
\midrule
$\text{mask}_m^j$ & The mask corresponding to the layer $j$ of the subnetwork $m$ \\
\midrule
$s_j$& The size of the kernel of the layer $j$\\
\midrule
$M$ & The number of subnetworks in an ensemble \\ 
\midrule
$\hat{\vy}^m_i$ & The prediction of the subnetwork number $m$ concerning the input $\vx_i$ \\ 
\midrule
$\hat{\vy}_i$ & The prediction of the ensemble concerning the input $\vx_i$ \\
\midrule
$\alpha$ & The width-augmentation factor of Packed-Ensembles \\ 
\midrule
$\gamma$ & The number of subgroups of Packed-Ensembles \\
\midrule
$\vtheta_{\alpha,m}$ & The set of weights of the subnetwork $m$ with a width factor $\alpha$ \\ 
\midrule
$\vomega^{j}_{\alpha, \gamma}$& The weights of layer $j$ with $\gamma$ groups and a width factor $\alpha$ \\
\bottomrule
\end{tabular}
}

\end{table*}

\clearpage

